Application of Deep Learning in Fundus Image Processing for Ophthalmic Diagnosis -- A Review

An overview of the applications of deep learning in ophthalmic diagnosis using retinal fundus images is presented. We also review various retinal image datasets that can be used for deep learning purposes. Applications of deep learning for segmentation of optic disk, blood vessels and retinal layer as well as detection of lesions are reviewed. Recent deep learning models for classification of diseases such as age-related macular degeneration, glaucoma,diabetic macular edema and diabetic retinopathy are also reported.

==> sections/applications/dme.tex <==
One of the first results on DME detection by deep learning using OCT images was presented by Chan et al \cite{chan2017transfer} using SERI dataset. The authors used Transfer Learning with AlexNet to extract features and classified images with SVM classifier. With 8 fold cross-validation it achieved 96\% accuracy.

Vahadane et al. \cite{vahadane2018detection} used patch based deep learning architecture for detecting diabetic macular edema by two step methods using Heidelberg OCT image data (Section \ref{data:hiedelberg}). In the first step image processing techniques were used to extract hard exudates, fluid filled region, retinal pigment epithelium. Then patch based CNN classifier was used to determine if the class was with DME or not. It achieved an F1 score of 0.9281 on the test dataset.

Perdomo et al. \cite{perdomo2018oct} presented end-to-end CNN architecture to classify diabetic macular edema and normal OCT images. The authors achieved 93.75\% accuracy with a margin of error 3.125\%. A 12 layer CNN was used after pre-processing (cropping and resizing) the images. The SERI database (private dataset) with 32 volume spectral domain OCT images were used for this work.

Varadarajan et al. \cite{varadarajan2018predicting} used Inception-v3 CNN architecture to train a model to predict the presence of diabetic macular edema without segmenting any specific layer from OCT images unlike other studies on OCT data. The model was trained with fundus photographs and corresponding OCT images were used for testing. Total 6039 images collected from Rajavithi Hospital Thailand were used to train the model and the final AUC was 0.89 , Sensitivity was 0.85 with specificity 0.8.

Chan et al. \cite{chan2018fusing} performed transfer learning with OCT images collected from  Chinese  University Hong  Kong (private dataset) to classify normal and diabetic macular edema images. Features collected from preprocessed images with ALexNet, VggNet, GoogleNet were combined to form the feature vector. The dimension was reduced using Principle Component Analysis algorithm. KNN, SVM, Random Forest classifiers were used and with the majority voting between the classifiers highest accuracy and specificity were 90.63\% and 93.75\% respectively which is very similar to the result presented in \cite{perdomo2018oct}.

%Overview of all the discussed literature in this section is given at Table 7.
%\import{sections/tables/}{dme.tex}

==> sections/applications/oct.tex <==
Roy et al. \cite{roy2017relaynet} was the first to propose end-to-end CNN based deep learning architecture to segment retinal layers from OCT images using DUKE (Section \ref{data:duke}). The proposed deep learning architecture, named as ReLayNet was inspired from U-Net \cite{ronneberger2015u} and DeConvNet \cite{noh2015learning} and consisted of encoder and decoder blocks followed by a classification layer. The OCT scans were width-wise sliced and the sliced data were augmented by spatial translation and horizontal flips. The DICE score was used to evaluate the performance of the model and it resulted in scores of 0.94 for NFL-IPL layer, 0.9 for ILM layer, 0.87 for INL layer.

With retinal images traditional methods were also used with CNNs such as \cite{burlina2016detection} \cite{maji2015deep}. Fang et al. \cite{fang2017automatic} proposed a novel framework for combining CNN and graph search algorithms to segment nine different layers found in retina OCT images. Here the CNN, trained using patches was used to extract features from the retinal boundaries initially and a classifier was trained to describe the retinal layer structures. Finally, the probability maps created from the CNN outputs were used to get the final boundary layers by graph search algorithms. One hundred seventeen spectral domain-OCT images with AMD were used to check the reliability of the model to segmentation the retinal layers from OCT images.

Unlike the patch-based method such as the one in \cite{fang2017automatic}, Ben-Cohen et al. \cite{ben2017retinal} proposed a different architecture where the loss function was calculated with full image context. The authors reported the application of U-Net based FCN to segment retinal layers of OCT images. Graph search approach along with Sobel filtering was implemented to detect boundary layers. The algorithm was validated on 24 patients of DME and epiretinal membrane and achieved satisfactory results. DICE coefficients were 0.5,0.94,0.85 for 3 different FCN architectures.

Pekala et al. \cite{pekala2018deep} used non-proliferative DR OCT images from 10 patients from University of Miami dataset. A novel feature of this work was the use of FCN based on DenseNet architecture and Gaussian process based regression. Per-pixel unsigned error was calculated using 10 fold cross validation and mean boundary estimation error was 1.07 with a standard deviation of 0.14. 

Motivated by previous results from combining  different deep learning architecture and conventional machine learning approaches, Liu et al. \cite{liu2018automated} proposed a method for retinal layer segmentation from OCT images using a combination of hand-crafted features and deep features which were extracted using a deep residual network. A random forest classifier was trained using these features and at the last step shortest path was calculated to get the final segmentation from the contour probability graph of each layer obtained from the trained classifier. This method used DUKE DME dataset (Section \ref{data:duke}) and achieved an F1 score of 0.885.


==> sections/applications/oct_amd.tex <==
AMD classification works has also been done with OCT images, few of them are described below.

Treder et al. \cite{treder2018automated} presented an application of deep learning in spectral domain OCT image (SD-OCT) classification for AMD detection using the Heidelberg Engineering dataset (Section \ref{data:hiedelberg}). The SD-OCT data from 701 AMD and 311 healthy patients were used for this multi-layer Deep CNN classification model. In an Inception-v3 network, the first layer was modelled as DCNN trained with millions of Imagenet database images and the last layers were trained with SD-OCT images for performing classification. After the first 500 steps, this model achieved an accuracy of 100\%.

Kermany et. al \cite{kermany2018identifying} used transfer learning on 51,140 normal, 8,617 drusen, 37,206 choroidal neovascularization and 11,349 diabetic macular edema images from a private database. The model was applied to 1,000 untrained OCT images for validation. It achieved a 100\% accuracy for classification between normal and choroidal neovascularization images whereas it was able to classify between diabetic macular edema and normal images with 98.2\% accuracy, and between normal and drusen images with 99\% accuracy.

==> sections/applications/oct_glaucoma.tex <==
Muhammad et al. \cite{muhammad2017hybrid} used a hybrid of AlexNet and random forest on wide field OCT of 102 patients for glaucoma classification. The pre-trained AlexNet model was used for feature extraction from OCT images. The weights of nodes of fully connected layers of the neural net were used as input for the random forest classifier. Six image types for each patient were used with leave-one-out cross-validation to train the model. A vertically flipped copy of each image was also added and nodes from fully connected layer 6 were found to have the best accuracy of 93.1\% using RNFL probability map. The method outperforms OCT and VF clinical metrics which gave up to 87.3\% accuracy but fell short of 98\% obtained by an experienced human expert. %These 6 images consist of (1) RGC + thickness map, (2) RNFL thickness map, (3) RGC + probability map, (4) RNFL probability map (5) en face projection and (6) Combination of (2), (3) and (4) in r, g and b channels respectively. 

%// Alexnet + random forests block diagram

Fu et. al.\cite{fu2018multi} presented multi-context deep network (MCDN) for angle-closure glaucoma screening using a private dataset called Visante Anterior Segment OCT dataset. Two parallel streams were used to fine-tune a pre-trained VGG-16 on the local and global image. The feature maps from these streams were concatenated at the dense layer and supplemented with clinical parameters with analysis by a linear SVM for final classification. Intensity-based data augmentation was performed instead of traditional scale based augmentation because the anterior chamber was found at a consistent position in AS-OCT images and obtained an AUC of 0.9456.

==> sections/datasets.tex <==
\section{Data Types and Datasets} \label{sec:datasets}
The various imaging datatype and datasets used in the literature are summarized herein.

\import{sections/}{fundus.tex}
\import{sections/datasets/}{achiko.tex}
\import{sections/datasets/}{areds.tex}
\import{sections/datasets/}{chase.tex}
\import{sections/datasets/}{cleo.tex}
\import{sections/datasets/}{diaretdb1.tex}
\import{sections/datasets/}{diaretdb0.tex}
\import{sections/datasets/}{drions.tex}
\import{sections/datasets/}{drishti.tex}
\import{sections/datasets/}{drive.tex}
\import{sections/datasets/}{eyepacs.tex}
\import{sections/datasets/}{hrf.tex}
\import{sections/datasets/}{kora.tex}
\import{sections/datasets/}{seed.tex}
\import{sections/datasets/}{stare.tex}
\import{sections/datasets/}{messidor.tex}
\import{sections/datasets/}{ophtha.tex}
\import{sections/datasets/}{ohnsd.tex}
\import{sections/datasets/}{origa.tex}
\import{sections/datasets/}{riga.tex}
\import{sections/datasets/}{rim.tex}
\import{sections/datasets/}{refuge.tex}
\import{sections/datasets/}{roc.tex}

\iffalse
\import{sections/}{oct.tex}
\import{sections/datasets/}{duke.tex}
\import{sections/datasets/}{heidelberg.tex}
\import{sections/datasets/}{noor.tex}
\import{sections/datasets/}{octid.tex}
\import{sections/datasets/}{ukb.tex}
\fi
% Table
% \import{sections/figures/}{datasets.tex}

==> sections/datasets/achiko.tex <==
\subsubsection{ACHIKO-K \cite{zhang2013achiko}} \label{data:achiko}
This database is dedicated mainly for glaucoma studies and was collected from a Korean population. In this database, there are 258 manually annotated fundus images among which 114 are glaucoma images and 144 are normal images. The online link to this dataset is \url{https://oar.a-star.edu.sg/jspui/handle/123456789/1080?mode=full}

==> sections/datasets/areds.tex <==
\subsubsection{AREDS \cite{clemons2003age}} \label{data:areds}
The \textit{Age-Related Eye Disease Study} (AREDS) is a database with 4757 AMD and non-AMD participants collected by National Eye Institute. In Nov 2010, the first part of this database came online with 72,000+ color fundus images from 595 participants. Later in 2014, 134,500+ images from 4,613 participants were added to it taking the total to above 206,500. This dataset can be obtained upon request and can be found at \url{https://www.ncbi.nlm.nih.gov/projects/gap/cgi-bin/study.cgi?study_id=phs000001.v3.p1}

==> sections/datasets/chase.tex <==
\subsubsection{CHASE \cite{owen2009measuring}} \label{data:chase}
The CHASE dataset retinal fundus image dataset is from the Child Heart and Health Study in England. It has 28 images with a resolution of 1280 X 960 pixels.

==> sections/datasets/cleo.tex <==
\subsubsection{CLEOPATRA \cite{sivaprasad2014multicentre}} \label{data:cleo}
It was a randomized study of patients with DR and DME to investigate significance of light mask in treatment of these diseases. This study was performed in UK with 15 patients. There are total 298 total images in the dataset captured with different types of cameras. This is not available publicly online.


==> sections/datasets/diaretdb0.tex <==
\subsubsection{DIARETDB0 \cite{kauppi2006diaretdb0}}  \label{data:diaretdb0}
This database was created for benchmarking DR from fundus images. There are 20 normal and 110 DR images. These images were acquired from Kuopio University Hospital in Finland. The online link to the dataset is \url{http://www.it.lut.fi/project/imageret/diaretdb0/}

==> sections/datasets/diaretdb1.tex <==
\subsubsection{DIARETDB1 \cite{kamarainen2007diaretdb1}}  \label{data:diaretdb1}
This dataset consists of 84 DR and 4 normal images which were acquired from Kuopio University Hospital in Finland captured with 50\degree\ FOV fundus camera. This dataset is online available at \url{http://www.it.lut.fi/project/imageret/diaretdb1/}

==> sections/datasets/drions.tex <==
\subsubsection{DRIONS-DB \cite{carmona2008identification}}  \label{data:drions}
This database consists of 110 color fundus images. Miguel Servet Hospital, Zaragossa Spain developed this dataset for optic nerve head segmentation. Among all the patients 23.1\%  had chronic glaucoma and 76.9\% of them had eye hypertension. This dataset can be found at \url{http://www.ia.uned.es/~ejcarmona/DRIONS-DB.html}

==> sections/datasets/drishti.tex <==
\subsubsection{DRISHTI-GS \cite{sivaswamy2015comprehensive} \cite{sivaswamy2014drishti}}  \label{data:drishti}
This fundus image database is mainly for OD and OC segmentation originated from CVIT Lab, IIT Hyderabad. There are 50 training images and 51 test images in the dataset. Ground truth for each image is available in the dataset. A fundus camera with a FOV of 30 \degree was used to collect the images. The dataset is publicly available at \url{http://cvit.iiit.ac.in/projects/mip/drishti-gs/mip-dataset2/Home.php}


==> sections/datasets/drive.tex <==
\subsubsection{DRIVE \cite{staal2004ridge}}  \label{data:drive}
DRIVE stands for \textit{Digital Retinal Images for Vessel Extractio}n. The database was obtained from a diabetic retinopathy screening program. It has 40 fundus images and 33 images are normal and 7 images are with mild diabetic retinopathy, captured with a Canon CR5 non-mydriatic 3CCD camera with a 45\degree \ field of view (FOV). The dataset is openly available at \url{https://www.isi.uu.nl/Research/Databases/DRIVE/}

==> sections/datasets/duke.tex <==
\subsubsection{DUKE Dataset \cite{farsiu2014quantitative}}  \label{data:duke}
This is publicly available OCT image database developed at DUKE University, Rayleigh NC consists of 269 AMD patients and 115 normal. The full dataset can be downloaded from \url{http://people.duke.edu/~sf59/RPEDC_Ophth_2013_dataset.htm}



==> sections/datasets/eyepacs.tex <==
\subsubsection{Kaggle/EyePACS \cite{niemeijer2010retinopathy}}  \label{data:eyepacs}
This dataset is from an online competition organized by Kaggle for DR detection. This dataset has 35,126 high-resolution fundus training images and 53,576 unlabelled test images. Images are in five groups: normal, mild, moderate, severe, proliferative. Clinician's rating for each image is provided. This dataset is available on registration at \url{https://www.kaggle.com/c/diabetic-retinopathy-detection/data}

==> sections/datasets/heidelberg.tex <==
\subsubsection{Heidelberg OCT database \cite{jahromi2014automatic}}  \label{data:hiedelberg}
This database is for corneal OCT images taken by Heidelberg imaging device. There are 15 images mainly dedicated for layer segmentation. This dataset can be found at \url{https://sites.google.com/site/hosseinrabbanikhorasgani/datasets-1/corneal-oct}


==> sections/datasets/hrf.tex <==
\subsubsection{HRF \cite{budai2013robust}}  \label{data:hrf}
This public database contains 15 images of healthy patients, 15 images of patients with DR and 15 images of glaucomatous patients captured with Canon CR-1 fundus camera with a 45\degree \ FOV. Expert segmentations are provided for each image. This can be found publicly at \url{https://www5.cs.fau.de/research/data/fundus-images/}

==> sections/datasets/kora.tex <==
\subsubsection{KORA \cite{brandl2016features}}  \label{data:kora}
The Cooperative Health Research in the Region of Augsburg, Germany developed this dataset to study AMD disease. Fundus images were collected from 2,840 patients. Link of this dataset is \url{https://epi.helmholtz-muenchen.de/.}
%\begin{longtable}[hbt!]
%\begin{center}
%\begin{adjustbox}{width=1\textwidth}


==> sections/datasets/messidor.tex <==
\subsubsection{MESSIDOR \cite{niemeijer2010retinopathy}} \label{data:messidor}
There are 1,200 images in MESSIDOR dataset captured with a color video 3CCD camera 45\degree \ FOV This retinal image dataset was created by three ophthalmology departments funded by the French Ministry of Research and Defense. Medical experts have provided the diagnosis for DR grade and ME risk for each image. The public link for this dataset is \url{http://www.adcis.net/en/Download-Third-Party/Messidor.html}. Recently A more updated version has come online and is called MESSIDOR-2 (\url{http://latim.univ-brest.fr/indexfce0.html} )

==> sections/datasets/noor.tex <==
\subsubsection{Noor Hospital OCT Database \cite{rasti2018macular}}  \label{data:noor}
This database was collected at Noor Hospital at Tehran. It consists of 50 DME, 50 normal and 48 AMD patients' OCT image data. The full dataset is available on \url{https://drive.google.com/file/d/1iSiFfD5LpLASrFUZu13uMFSRcFEjvbSq/view}

==> sections/datasets/octid.tex <==
\subsubsection{OCTID \cite{gholami2018octid}}  \label{data:octid}
This is an open-access huge OCT database with more than 500 OCT images collected from Sankara Nethralya Eye Hospital, Chennai, India. This database includes normal, macular hole, AMD, central serous retinopathy, and DR. Ground truth labels are provided for 25 images. The images are available publicly \url{https://dataverse.scholarsportal.info/dataverse/OCTID}


==> sections/datasets/ohnsd.tex <==
\subsubsection{ONHSD \cite{lowell2004optic}}  \label{data:onhsd}
This fundus image database was also developed for proper optic nerve head segmentation. Ninety-nine fundus images were acquired from a diabetic retinopathy screening program. The fundus camera used for this work was a Canon CR6 45MNf with a 45\degree \ FOV. The link for this dataset is \url{http://www.aldiri.info/Image%20Datasets/ONHSD.aspx}


==> sections/datasets/ophtha.tex <==
\subsubsection{e-optha \cite{decenciere2013teleophta}}  \label{data:eoptha}
This dataset consists of fundus images for Diabetic retinopathy research. This dataset has mainly two parts: one for exudates with 47 images with exudates, 35 images with no exudates; and another for MA with 233 normal images and 148 MA images. The full dataset is available at \url{http://www.adcis.net/en/Download-Third-Party/E-Ophtha.html}

==> sections/datasets/origa.tex <==
\subsubsection{ORIGA \cite{zhang2010origa}}  \label{data:origa}
ORIGA stands for \textit{Online Retinal Image dataset for Glaucoma Analysis}, and it consists of 650 retinal fundus images. The Singapore Eye Research Institute conducted the project and data were collected from the Singapore Malay Eye Study or SiMES over a three year period of 2004-2007. This dataset is not currently available online

==> sections/datasets/refuge.tex <==
\subsubsection{REFUGE \cite{refuge}}  \label{data:refuge}
This dataset is part of the retinal fundus glaucoma challenge organized by Medical Image Computing and Computer Assisted Intervention 2018 meeting held in Spain. This dataset has 1,200 annotated fundus Images. Recently this competition also included images for AMD. This can be found at \url{https://refuge.grand-challenge.org/} 


==> sections/datasets/riga.tex <==
\subsubsection{RIGA \cite{almazroa2018retinal}}  \label{data:riga}
RIGA stands for \textit{Retinal Images for Glaucoma Analysis}. This dataset mainly consists of retinal fundus images of glaucoma patients. The RIGA dataset was developed by concatenating images from MESSIDOR (Section \ref{data:messidor}), and images obtained from Magrabi Eye Centre, Riyadh and Bin Rashid Ophthalmic Centre, Riyadh. There are a total of 760 retinal fundus images in the database. This public dataset is now available online as \url{https://deepblue.lib.umich.edu/data/concern/generic_works/3b591905z}

==> sections/datasets/rim.tex <==
\subsubsection{RIM-ONE \cite{fumero2011rim}}  \label{data:rimone}
This retinal image database is mainly focused on optic nerve head segmentation. Its initial version consisted of 169 fundus images and segmentation annotations for each image. Subsequently, version r2 consisting of 455 images and version r3 consisting of 159 images were added. A Nidek AFC-210 Canon EOS 5D Mark II was used to capture the images in this project. This dataset is not currently available publicly.

==> sections/datasets/roc.tex <==
\subsubsection{Retinopathy Online Challenge \cite{niemeijer2010retinopathy}} \label{data:roc}
Retinopathy Online Challenge is a database for DR detection using CAD systems. A total of 100 fundus photographs taken with different cameras (Topcon NW 100, Topcon NW 200, Canon CR5-45NM cameras) are available in the dataset. Currently, the data annotations are not available but the images are available upon registration at \url{http://webeye.ophth.uiowa.edu/ROC/} 

==> sections/datasets/seed.tex <==
\subsubsection{SEED \cite{zheng2013much}}  \label{data:seed}
This database originated from a study performed by the Singapore Epidemiology of Eye Diseases. This dataset has 235 fundus images among which 43 are glaucoma images, 192 are normal images. This is not available online for public use. Singapore Chinese Eye Study (SCES) and Singapore Indian Eye Study (SINDI) databases also came out from this same study.


==> sections/datasets/seri.tex <==
\subsubsection{SERI \cite{lemaitre2016seri}} \label{data:seri}

==> sections/datasets/stare.tex <==
\subsubsection{STARE \cite{hoover2000locating}, \cite{hoover2003locating}}  \label{data:stare}
The \textit{Structured Analysis of the Retina} (STARE) dataset is a collection of 400 fundus images with blood vessel annotation only on 40 images captured by a TRV50 fundus camera with 35\degree \ FOV. The dataset is publicly available at \url{http://cecas.clemson.edu/~ahoover/stare/}

==> sections/datasets/ukb.tex <==
\subsubsection{UK BioBank \cite{mitry2013crowdsourcing}}  \label{data:ukb}
UK Biobank is a major health resource organization aims to improve the diagnosis and treatment of different kinds of diseases and not just ophthalmic cases. The biobank has 231,806 OCT and fundus files, along with various types of medical data. This dataset is available upon purchase from \url{https://www.ukbiobank.ac.uk}



==> sections/figures/ann.tex <==
\begin{figure}[hbt!]
\caption{Feed Forward Neural Network with 2 hidden layers}
\includegraphics[width=\textwidth]{media/feed-forward}\\
\end{figure}



==> sections/figures/conv-op.tex <==
\begin{figure}[hbt!]
\caption{An example of Convolution} 
\includegraphics[width=10cm]{media/conv-op}\\
\end{figure}


==> sections/figures/conv.tex <==
\begin{figure}[h]
\caption{Activations of CNN layers[refer cs231n]} 
\includegraphics[width=\textwidth]{media/conv}\\
\end{figure}


==> sections/figures/oct.tex <==
\begin{figure}[htb!]
\centering
\includegraphics[width=1\linewidth]{media/eye_oct.png}
\caption{OCT image including anatomy \cite{leopold_2017}.}
\label{fig:oct}
\end{figure}

==> sections/figures/relu.tex <==
\begin{figure}[h]
\caption{ReLU (Left) and Leaky ReLU (Right)} 
\includegraphics[width=\textwidth]{media/activation-fn}\\
\end{figure}


==> sections/fundus.tex <==
% \subsection{Different Retinal Imaging Techniques} \label{sec:tech}
\subsection{Fundus Imaging Technique}  \label{sec:tech_fundus}
Fundus imaging is the commonly used imaging technique to capture retinal images. `Fundus images are taken using fundus camera which is nothing but a low power microscope  to capture magnified and upright view of the fundus, Figure \ref{fig:fundus} shows retinal morphologies - i.e. optic disc and macula regions - and pathologies in a fundus image.

\import{sections/figures/}{fundus.tex}

%\subsubsection{Optical Coherence Tomography} \label{sec:tech_oct}
%Optical coherence tomography (OCT) is an important technique which is used frequently in retinal image analysis, as well as in non-destructive testing and cardiology. The optical principle of OCT is based on low coherence interferometry: by applying near-infrared light, this imaging technique can capture micrometer high-resolution images \cite{roy2018automated}. Sample OCT image with labeling is shown in Figure \ref{fig:oct}.

%\import{sections/figures/}{oct.tex}

==> sections/kpis.tex <==
\section{Performance Measures} \label{sec:kpis}
Possible outcomes for any classification outcome of any sample
1. True Positive (TP): Positive sample classified as positive.
2. False Positive (FP): Negative sample classified as positive.
3. True Negative (TN): Negative sample classified as negative.
4. False Negative (FN): Positive sample classified as negative.
In this section mostly used performance measures of any algorithm are discussed in brief below.
\subsection{Sensitivity}
This is the proportion of positive results which are classified properly as positive. Mathematically this can be written as \ TP/(TP+FN)\
\subsection{Specificity}This is the proportion of negative results which are classified properly as negative. Mathematically this can be written as \ TN/(TN+FP)\
%\subsection{AUC}
\subsection{ROC}
ROC curve, is a graphical plot between TP Rate and FP rate and Area Under Curve (AUC) means the area under the curve.It signifies the probability of a model to classify more positive than negative.
\subsection{DICE Coefficient}
This is the similarity index between two samples.It is also called F1 score. Mathematically it can be written as \ 2TP/(2TP+FP+FN)\
%\subsection{F1 Score}


==> sections/oct.tex <==
\subsection{Optical Coherence Tomography} \label{sec:tech_oct}
Optical coherence tomography (OCT) is an important technique which is used frequently in retinal image analysis among other applications. The optical principle of the OCT is based on low coherence interferometry with near IR light \cite{fercher2003optical} , this imaging technique can capture micro level high resolution images. Sample OCT image with labeling is shown in Figure \ref{fig:oct}.

\import{sections/figures/}{oct.tex}

==> sections/tables/amd.tex <==
\begin{table}[hbt!]
\caption {Summary of AMD Detection Works} \label{tab:title}
%\begin{adjustbox}{width=1\textwidth}
 \begin{adjustbox}{width=1\textwidth}
%\resizebox{1.3\textwidth}{!}{
\begin{tabular}{m{2.5cm}m{2cm}m{2.5cm}m{2.5cm}m{2.5cm}m{2.5cm}m{2.5cm}m{2.5cm}m{2.5cm}}
%\tabcolsep=0.1cm
\hline
\textbf{Reference} & \textbf{Modality} & \textbf{ Architecture} & \textbf{Dataset} & \textbf{Acc} & \textbf{SN} & \textbf{SP} & \textbf{AUC}\\
\hline
Grassmann et al. & fundus & CNN using AlexNet, GoogleNet, VGG, ResNet, Inception-v3, 1-ResNet-v2 & AREDS and KORA & 94.3\% \\ \hline
Horta et al. & fundus & DCNN & AREDS & 79.04\% & 66.34\% & 88.95\% & .8476 \\ \hline
Burlina et al. & fundus & Deep Features with SVM & AREDS & 93.4\% & & &\\ \hline
Burlina et al. & fundus & DCNN using AlexNet & AREDS & 91.6\%& & & .96\\ \hline
Govindaiah et al. & fundus & VGG16 & AREDS dataset &92.5\% \\ \hline
Matsuba et al. & fundus & DCNN & Tsukazaki  Hospital & 100\% &100\%& 97.31\%& .9976 \\ \hline
HongTan et al. & fundus & CNN & Kasturba Medical College & 95.45\% & 96.43\% & 93.45\% \\ \hline
Treder et al. & SD-OCT & 701 AMD, 311 healthy & CNN using Inception-v3 & 96\% & 100\% & 92\% \\ \hline
Kermany et al. & OCT & Transfer Learning & 51140 normal, 8617 drusen, 37206 CNV, 11349 DME & 96.6\% & 97.8\% & 97.4\% & .999 \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}

==> sections/tables/dme.tex <==
\begin{table}[hbt!]
\caption {Summary of DME Detection Works} \label{tab:title}
\begin{adjustbox}{width=1\textwidth}
%\resizebox{1.3\textwidth}{!}{
\begin{tabular}{m{2.5cm}m{2cm}m{2.5cm}m{2.5cm}m{2cm}m{2cm}m{2cm}m{2cm}}
%\tabcolsep=0.1cm
\hline
\textbf{Reference} & \textbf{Imaging Modality} & \textbf{Architecture} & \textbf{Dataset} & \textbf{Acc} & \textbf{SN} & \textbf{SP} & \textbf{F1 Score}\\
\hline
Chan et al. & OCT & CNN features+ Majority voting& SERI& 93.75\%& 93.75\&&93.75\%\\ \hline
Vahadan et al. & OCT & patchbased CNN & Heidelberg & & & & 0.9281 \\ \hline
Varadarajan et al. & OCT & Rajavithi Hospital Thailand & CNN Inception v-3 & 85\% & 80\% & 89\%\\ \hline
Perdomo et al. & OCT & SERI & CNN & 93.75\% \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}

==> sections/tables/dr.tex <==
\begin{table*}[hbt!]
\caption {Summary of Diabetic Retinopathy Detection Works} \label{tab:title}
\begin{adjustbox}{width=1\textwidth}
%\resizebox{1.3\textwidth}{!}{
\begin{tabular}{m{2.5cm}m{2cm}m{2.5cm}m{2.5cm}m{2.5cm}m{2.5cm}m{2.5cm}m{2.5cm}m{2.5cm}}
%\tabcolsep=0.1cm
\hline
\textbf{Reference} & \textbf{Modality} & \textbf{Architecture} & \textbf{Dataset} & \textbf{Acc} & \textbf{SN} & \textbf{SP} & \textbf{AUC} \\
\hline
Gargeya et al. & fundus & CNN Deep Residual Learning & EyePACS, MESSIDOR e-Optha2 & & 94\% & 98\% & .97 \\ \hline
Takahashi et al. & fundus & CNN GoogleNet, ResNet & 9839 images & 96\% \\ \hline
Colas et al.& fundus & CNN & EyePACS & & 96.2\% & 66.6\% & .946\\ \hline
Garcia et al. & fundus & CNN AlexNet & EyePACS & 83.68\% & & 93.65\%  \\ \hline
%Desbiens et al.&
Abramoff et al. & fundus &  CNN AlexNet & Messidor-2 & & 96.8\% & 87\% \\ \hline
Brown et al. & fundus & CNN GoogleNet, U-Net, Transfer Learning & Private: 6000 images & & 96.8\% & 87\% & .98 \\ \hline
Gulshan et al. & fundus & CNN Incetionv-3 & EyePACS-1, Messidor-2 & & 90.3\%, 87\% & 98.1\%, 98.5\% & .99, .99 \\ \hline
Quellec et al. & fundus & ConvNet & Kaggle, e-optha, DiaretDB1 & & & & .954, .949, .955 \\ \hline  

\end{tabular}
%}
%\end{center}
\end{adjustbox}
\end{table*}

==> sections/tables/glauc.tex <==
\begin{table}
\caption {Summary of Glaucoma Detection Works} \label{tab:title}
%\begin{center}
\begin{adjustbox}{width=1\textwidth}
%\resizebox{1.3\textwidth}{!}{
\begin{tabular}{m{2.5cm}m{2cm}m{2.5cm}m{2.5cm}m{2.5cm}m{2.5cm}m{2.5cm}m{2.5cm}m{2.5cm}}
\hline
\textbf{Reference} & \textbf{Modality} & \textbf{Architecture} & \textbf{Dataset} & \textbf{Acc} & \textbf{SN} & \textbf{SP} & \textbf{AUC}\\ \hline
%\tabcolsep=0.1cm
Asoaka et al. &fundus&3 layer FNN & Private: 171& & & &.926 \\ \hline
Zhixi et al. &fundus & Inception-v3 & Private:48000+ & & 95.6\%& 92.0\%& .986\\ \hline
Chen et al. &fundus &  4 layer CNN & ORIGA, SCES && & & .831, .887 \\ \hline
Chen et al. &fundus & C-CNN & ORIGA, SCES && & & .838, .898\\ \hline
Chai et al. &fundus & MB-NN & Private: 2554 &91.51\% & 92.33\% & 90.90\%& \\ \hline
Fu et al. &fundus & DENet & SCES, SINDI & 83.2\%, 66.6\% & & 70.67\%, 37.53\%\\ \hline
Chakravarty et al. & fundus &  Multi-task CNN & REFUGE &&&& .95 \\ \hline
Muhammad et al. & OCT & HDLM & Private:102 images & 93.1\%  \\ \hline
Fu et al. & OCT & MCDN  & Private:8270 images & 89.26\% & 88.89\% & 89.63\% &.9456 \\ \hline
\end{tabular}
\end{adjustbox}

\end{table}

==> sections/tables/ma.tex <==
\begin{table}[hbt!]
\caption {Summary of Red Lesion Detection Works} \label{tab:title}
%\begin{center}
\begin{adjustbox}{width=1\textwidth}
%\resizebox{1.3\textwidth}{!}{
\begin{tabular}{m{2.5cm}m{2cm}m{2.5cm}m{2.5cm}m{2.5cm}m{2.5cm}m{2.5cm}m{2.5cm}}
%\tabcolsep=0.1cm
\hline
\textbf{Reference} & \textbf{Modality} & \textbf{Architecture} & \textbf{Dataset} & \textbf{Acc} & \textbf{SN} & \textbf{SP} & \textbf{AUC} \\ \hline

Orlando et al. & fundus & CNN using LeNet architecture & e-optha, MESSIDOR & & & & .8812, .8932 \\ \hline
Grinsven et al.& fundus & CNN using OxfordNet & MESSIDOR, EyePACS & & 91.9\%, 83.7\% & 91.8\%, 85.1\% & .972, .895\\ \hline
%Carson et al. & fundus & CNN using GoogleNet, ResNet, VGG16, AlexNet, Inception-v3 & EyePACS, e-optha & Acc 98\% \\ \hline
Lam et al. & fundus & CNN using GoogleNet3 & EyePACS, e-optha & 98\% & & & .95\\ \hline
%Shan et al. & fundus & SSAE & DIARETDB & 91.38\% & & .916\\ \hline
Shan et al. & fundus & Transfer Learning (SSAE) & DIARETDB &  91.38\% & & & .916\\ \hline
Haloi & fundus & 5 layer CNN & MESSIDOR, ROC & 96\% & 97\% & 96\%& .982, .98 \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}

==> sections/tables/mergedtable.tex <==
\begin{sidewaystable}
% \begin{table}
\caption {Summary of works using deep learning for ophthalmic diagnosis} \label{tab:summary}
%\begin{center}
\begin{adjustbox}{width=1\textwidth}
%\resizebox{1.3\textwidth}{!}{
\begin{tabular}{m{3cm}m{4cm}m{2cm}m{6cm}m{6cm}m{3.5cm}m{3.5cm}m{3.5cm}m{3.5cm}m{3.5cm}}
%\tabcolsep=0.1cm
\hline
\textbf{Application} & \textbf{Reference} & \textbf{Modality} & \textbf{Architecture} & \textbf{Dataset} & \textbf{Acc} & \textbf{SN} & \textbf{SP} & \textbf{AUC} & \textbf{F1} \\
\hline
%Camino et al. & fundus & CNN using MatConvNet & 304 Private OCT & 91.2\% similarity with human annotation \\ \hline
\multirow{10}{*}{\textbf{OD Seg}}& Lim et al.& fundus & 3-class CNN & MESSIDOR, SEED-DB &  &  &  & .847\\ \cline{2-10} 
& Maninis et al. & fundus & CNN DRIU & DRIVE, STARE, DRIONS-DB, RIM-ONE &  &  &  &  & .822, .831, .971, .959 \\ \cline{2-10}
& Feng et al. & fundus & FCN & DRIONS-DB & & 93.12\% & 99.56\% & & .9093\\ \cline{2-10}
&Sevastopolsky & fundus & U-net & RIM-ONE (OD, OC), DRIONS-DB (OD),DRISHTI-GS &  0.95, 0.82, 0.94, 0.85 &&&& \\ \cline{2-10}
& Edupuganti et al. & fundus & VGG16 FCN & Drishti-GS &  &  &  &  & .967  \\ \cline{2-10}
& Al-Bander et al. & fundus & CNN & Messidor (OD, Fovea)& 97\%, 96.6\% &  &  &  &   \\ \cline{2-10}
 & Mitra et al. & fundus & CNN & MESSIDOR, EyePACS & 99.05\%, 98.78\% &  & 99.14\%, 98.17\% &  & \\ \cline{2-10}
%Jen Hong Tan et al. & CNN &  & \\ \hline
& Liu et al. & fundus & ResNet50 FCN & 3 centres from Sydney, HRF, RIM-ONE & 91.6\% & 87.9\% & 96.5\% & .97\\ \hline


\multirow{5}{*}{\textbf{Lesion Seg}} & Haloi & fundus & 5 layer CNN & MESSIDOR, ROC & 96\% & 97\% & 96\%& .982, .98 &\\ \cline{2-10}
& Shan et al. & fundus & Transfer Learning (SSAE) & DIARETDB &  91.38\% & & & .916 &\\ \cline{2-10}
& Grinsven et al.& fundus & CNN using OxfordNet & MESSIDOR, EyePACS & & 91.9\%, 83.7\% & 91.8\%, 85.1\% & .972, .895 &\\ \cline{2-10}
& Tan et al. & fundus & 10 layer CNN & CLEOPATRA & & .8758 & .7158 & &\\ \cline{2-10}
& Orlando et al. & fundus & CNN using LeNet architecture & e-optha, MESSIDOR & & & & .8812, .8932 &\\ \cline{2-10}
%Carson et al. & fundus & CNN using GoogleNet, ResNet, VGG16, AlexNet, Inception-v3 & EyePACS, e-optha & Acc 98\% \\ \hline
 & Lam et al. & fundus & CNN using GoogleNet3 & EyePACS, e-optha & 98\% & & & .95 &\\ \hline
%Shan et al. & fundus & SSAE & DIARETDB & 91.38\% & & .916\\ \hline


\multirow{8}{*}{\textbf{Vessel Seg}} & Maji et al. & fundus & RF and DNN & DRIVE & 93.27\% & & & .9195&\\ \cline{2-10}
 & Liskowski et al. & fundus & CNN & DRIVE, STARE, CHASE\_DB & 97\% & & & .99&\\ \cline{2-10}
 & Melinscak et al.. & fundus & MPCNN & DRIVE & 94.66\% & & & .9749&\\ \cline{2-10}
 & Maji et al. & fundus & ConvNet ensemble & DRIVE & 94.7\% & & & .9283 &\\ \cline{2-10}
 & Fu et al. & fundus & FCN, CRF & DRIVE, STARE & 94.70\%, 95.45\% & .7294, .7140 & & &\\ \cline{2-10}
& Leopold et al. & fundus & FCN using RETSEG13 & DRIVE & 94.78\% & 68.23\% & 98.01\% & .9707&\\ \cline{2-10} 
& Zhang et al. & fundus & CNN(U-Net) & DRIVE, STARE, CHASE\_DB1 & 95.04\%, 97.12\%, 97.7\% & 87.23\%, 76.73\%, 76.7\% & 96.18\%, 99.01\%, 99.09\% & .9799, .9882, .99 &\\ \cline{2-10}
 & Oliveira et al. & fundus & CNN & DRIVE, STARE, CHASE\_DB1 & 95.76\%, 96.94\%, 96.53\% & 80.39\%, 83.15\%, 77.79\% & 98.04\%, 98.58\%, 98.64\% & .9821, .9905, .9855&\\ \cline{2-10}
 & Liu et al. & fundus & Densely Connected CNN & DRIVE & 95\% &\\ \cline{2-10}
 & Hu et al. & fundus & CNN(VGG-16 model) & DRIVE,STARE & 95.33\%, 96.32\% \\ \hline


\multirow{8}{*}{\textbf{AMD}}
& Burlina et al. & fundus & Deep Features with SVM & AREDS & 93.4\% & & & &\\ \cline{2-10}
 & Burlina et al. & fundus & DCNN using AlexNet & AREDS & 91.6\%& & & .96 &\\ \cline{2-10}
 & Horta et al. & fundus & DCNN & AREDS & 79.04\% & 66.34\% & 88.95\% & .8476 &\\ \cline{2-10}
& Govindaiah et al. & fundus & VGG16 & AREDS dataset &92.5\% & \\ \cline{2-10} 
& Matsuba et al. & fundus & DCNN & Tsukazaki  Hospital & 100\% &100\%& 97.31\%& .9976 & \\ \cline{2-10}
& Tan et al. & fundus & CNN & Kasturba Medical College & 95.45\% & 96.43\% & 93.45\% & \\ \cline{2-10}
& Grassmann et al. & fundus & Various CNN & AREDS, KORA & 94.3\% &\\ \hline

\multirow{7}{*}{\textbf{Glaucoma}}
& Chen et al. &fundus &  6 layer CNN & ORIGA, SCES && & & .831, .887 & \\ \cline{2-10}
& Chen et al. &fundus & C-CNN & ORIGA, SCES && & & .838, .898 & \\ \cline{2-10}
& Asoaka et al. &fundus&3 layer FNN & Private: 171& & & &.926 & \\ \cline{2-10}
& Fu et al. &fundus & DENet & SCES, SINDI & 83.2\%, 66.6\% & & 70.67\%, 37.53\% & \\ \cline{2-10}
& Chakravarty et al. & fundus &  Multi-task CNN & REFUGE &&&& .95 & \\ \cline{2-10}
& Zhixi et al. &fundus & Inception-v3 & Private:48000+ & & 95.6\%& 92.0\%& .986 & \\ \cline{2-10}
& Chai et al. &fundus & MB-NN & Private: 2554 &91.51\% & 92.33\% & 90.90\%& & \\ \hline

\multirow{9}{*}{\textbf{DR}}& Abramoff et al. & fundus &  CNN AlexNet & Messidor-2 & & 96.8\% & 87\% \\ \cline{2-10}
& Colas et al.& fundus & CNN & EyePACS & & 96.2\% & 66.6\% & .946\\ \cline{2-10}
& Gulshan et al. & fundus & Incetionv-3 & EyePACS-1, Messidor-2 & & 90.3\%, 87\% & 98.1\%, 98.5\% & .99, .99 \\ \cline{2-10}
& Gargeya et al. & fundus & CNN Deep Residual Learning & EyePACS, MESSIDOR e-Optha2 & & 94\% & 98\% & .97 \\ \cline{2-10}
& Quellec et al. & fundus & ConvNet & Kaggle, e-optha, DiaretDB1 & & & & .954, .949, .955 \\ \cline{2-10} 
& Takahashi et al. & fundus & CNN GoogleNet, ResNet & 9839 images & 96\% \\ \cline{2-10}
& Garcia et al. & fundus & CNN AlexNet & EyePACS & 83.68\% & & 93.65\%  \\ \hline


\multirow{6}{*}{\textbf{Layer Seg}} & Roy et al. & OCT & FCN & DUKE &  & .94 &\\ \cline{2-10}
 & Fang et al. & OCT & CNN & 117 SD-OCT & 1.26 mean, 1.24 SD &\\ \cline{2-10}
 & Ben-Cohen et al. & fundus & Patchbased U-Net,  OCTexplorer  &  TASMC(private) &  &  .95, .94, .85(RNFL) & \\ \cline{2-10}
 & Pekala et al. & OCT & FCNN & 50 OCT U. of Miami & Mean error 1.1 & \\ \cline{2-10}
 & Liu et al.& OCT & Deep Residual Network & DUKE  & & .885 & \\ \hline
 

\multirow{4}{*}{\textbf{DME}} & Chan et al. & OCT & CNN, Majority voting& SERI& 93.75\%& 93.75\&&93.75\%\\ \cline{2-10}
 & Vahadan et al. & OCT & patchbased CNN & Heidelberg & & & & & 0.9281 \\ \cline{2-10}
 & Varadarajan et al. & OCT & Rajavithi Hospital Thailand & CNN Inception v-3 & 85\% & 80\% & 89\%\\ \cline{2-10}
 & Perdomo et al. & OCT & SERI & CNN & 93.75\% \\ \hline


\multirow{2}{*}{\textbf{AMD}}& Treder et al. & OCT & 701 AMD, 311 healthy & CNN using Inception-v3 & 96\% & 100\% & 92\% \\ \cline{2-10}
& Kermany et al. & OCT & Transfer Learning & 51140 normal, 8617 drusen, 37206 CNV, 11349 DME & 96.6\% & 97.8\% & 97.4\% & .999 & \\ \hline

\multirow{2}{*}{\textbf{Glaucoma}}& Muhammad et al. & OCT & HDLM & Private:102 images & 93.1\% & \\ \cline{2-10}
& Fu et al. & OCT & MCDN  & Private:8270 images & 89.26\% & 88.89\% & 89.63\% &.9456 & \\ \hline

\end{tabular}
\end{adjustbox}
% \end{table}
\end{sidewaystable}


==> sections/tables/od.tex <==
\begin{table}[hbt!]
\caption {Summary of Some Optic Disc Segmentation Results} \label{tab:title}
%\begin{center}
\begin{adjustbox}{width=1\textwidth}
%\resizebox{1.3\textwidth}{!}{
\begin{tabular}{m{2.5cm}m{2cm}m{2.5cm}m{2.5cm}m{2cm}m{2cm}m{2cm}m{2cm}m{2cm}}
%\tabcolsep=0.1cm
\hline
\textbf{Reference} & \textbf{Modality} & \textbf{Architecture} & \textbf{Dataset} & \textbf{Acc} & \textbf{SN} & \textbf{SP} & \textbf{AUC} & \textbf{F1 Score} \\
\hline
%Camino et al. & fundus & CNN using MatConvNet & 304 Private OCT & 91.2\% similarity with human annotation \\ \hline
Mitra et al. & fundus & CNN & MESSIDOR, EyePACS & 99.05\%, 98.78\% &  & 99.14\%, 98.17\% &  & \\ \hline
Edupuganti et al. & fundus & VGG16 FCN & Drishti-GS &  &  &  &  & .967  \\ \hline
%Jen Hong Tan et al. & CNN &  & \\ \hline
Maninis et al. & fundus & CNN DRIU & DRIVE, STARE, DRIONS-DB, RIM-ONE &  &  &  &  & .822, .831, .971, .959 \\ \hline
Lim et al.& fundus & 3-class CNN & MESSIDOR, SEED-DB &  &  &  & .847\\ \hline 
Liu et al. & fundus & ResNet50 FCN & 3 centres from Sydney, HRF, RIM-ONE & 91.6\% & 87.9\% & 96.5\% & .97\\ \hline
Feng et al. & fundus & FCN & DRIONS-DB & & 93.12\% & 99.56\% & & 0.9093\\ \hline
\end{tabular}
\end{adjustbox}
\end{table}

==> sections/tables/retseg.tex <==
\begin{table}[hbt!]
\caption {Summary of Retinal Layer Segmentation Works} \label{tab:title}
%\begin{center}
\begin{adjustbox}{width=1\textwidth}
%\resizebox{1.3\textwidth}{!}{
\begin{tabular}{m{3cm}m{3cm}m{3cm}m{3cm}m{3cm}m{3cm}}
%\tabcolsep=0.1cm
\hline
\textbf{Reference} & \textbf{Modality} & \textbf{Architecture} & \textbf{Dataset} & \textbf{Acc} & \textbf{F1 Score}\\ \hline
Roy et al. & OCT & FCN & DUKE &  & .94\\ \hline
Fang et al. & OCT & CNN & 117 SD-OCT & 1.26 mean, 1.24 SD \\ \hline
Pekala et al. & OCT & FCNN & 50 OCT U. of Miami & Mean error 1.1 \\ \hline
Ben-Cohen et al. & fundus & Patchbased U-Net FCN,  OCTexplorer  &  TASMC(private) &  &  .95, .94, .85(RNFL) \\ \hline
Liu et al.& OCT & Deep Residual Network & DUKE  & & .885 \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}

==> sections/tables/summary.tex <==
\begin{table*}[hbt!]
\caption {Summary Table} \label{tab:summary}
\begin{adjustbox}{width=1\textwidth}
%\resizebox{1.3\textwidth}{!}{
\begin{tabular}{m{2.5cm}m{2cm}m{2.5cm}m{2.5cm}m{2cm}m{2cm}m{2cm}m{2cm}m{2cm}}
%\tabcolsep=0.1cm
\hline
\textbf{Reference} & \textbf{Modality} & \textbf{Architecture} & \textbf{Dataset} & \textbf{Acc} & \textbf{SN} & \textbf{SP} & \textbf{AUC} & \textbf{F1 Score}\\
\hline
Gargeya et al. & fundus & CNN Deep Residual Learning & EyePACS, MESSIDOR e-Optha2 & & 94\% & 98\% & .97 \\ \hline  

\end{tabular}
%}
%\end{center}
\end{adjustbox}
\end{table*}

==> sections/tables/vesseg.tex <==
\begin{table}[hbt!]
\caption {Summary of Retinal Blood Vessel Segmentation Results} \label{tab:title}
%\begin{center}
\begin{adjustbox}{width=1\textwidth}
%\resizebox{1.3\textwidth}{!}{
\begin{tabular}{m{2.5cm}m{2cm}m{2.5cm}m{2.5cm}m{2.5cm}m{2.5cm}m{2.5cm}m{2.5cm}}
%\tabcolsep=0.1cm
\hline
\textbf{Reference} & \textbf{Modality} & \textbf{Architecture} & \textbf{Dataset} & \textbf{Acc} & \textbf{SN} & \textbf{SP} & \textbf{AUC} \\ \hline

Zhang et al. & fundus & CNN(U-Net) & DRIVE, STARE, CHASE\_DB1 & 95.04\%, 97.12\%, 97.7\% & 87.23\%, 76.73\%, 76.7\% & 96.18\%, 99.01\%, 99.09\% & .9799, .9882, .99\\ \hline
Oliveira et al. & fundus & CNN & DRIVE, STARE, CHASE\_DB1 & 95.76\%, 96.94\%, 96.53\% & 80.39\%, 83.15\%, 77.79\% & 98.04\%, 98.58\%, 98.64\% & .9821, .9905, .9855\\ \hline
Liu et al. & fundus & Densely Connected CNN & DRIVE & 95\% \\ \hline 
Leopold et al. & fundus & FCN using RETSEG13 & DRIVE & 94.78\% & 68.23\% & 98.01\% & .9707\\ \hline
Liskowski et al. & fundus & CNN & DRIVE, STARE, CHASE\_DB & 97\% & & & .99\\ \hline
Maji et al. & fundus & RF and DNN & DRIVE & 93.27\% & & & .9195\\ \hline
Maji et al. & fundus & ConvNet ensemble & DRIVE & 94.7\% & & & .9283 \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}

